Certifiably Robust Image Watermark

Generative AI raises many societal concerns such as boosting disinformation and propaganda campaigns. Watermarking AI-generated content is a key technology to address these concerns and has been widely deployed in industry. However, watermarking is vulnerable to removal attacks and forgery attacks. In this work, we propose the first image watermarks with certified robustness guarantees against removal and forgery attacks. Our method leverages randomized smoothing, a popular technique to build certifiably robust classifiers and regression models. Our major technical contributions include extending randomized smoothing to watermarking by considering its unique characteristics, deriving the certified robustness guarantees, and designing algorithms to estimate them. Moreover, we extensively evaluate our image watermarks in terms of both certified and empirical robustness. Our code is available at \url{https://github.com/zhengyuan-jiang/Watermark-Library}.

==> 6_discussion.tex <==
% \section{Discussion and Limitations}
% \myparatight{Text \& audio watermarking} Actually, we can obtain the certified robustness guarantee for any watermarking method that uses a bitstring as the watermark. In our work, we only conduct experiments for image watermarking. For audio watermarking, the original signal are first transformed into STFT spectrogram, and the watermark is embedded into the spectrogram by methods similar to image watermarking. Then, the spectrogram is transformed back to the watermarked signal via inverse STFT. To use our method, we can add gaussian noises sampled uniformly at random in the spectrogram space, and derive certified robustness guarantees using our smoothing variants. Specifically, no matter how an audio signal is modified, as long as the distance between perturbed signal and original signal in the spectrogram is $\ell_2$-norm bounded by a certain value, the pertrubed watermarked signal's bitwise accuracy will be bounded by a lower and upper bound. We notice that existing work~\cite{liu2023dear,liu2023detecting} still use $\ell_2$-norm distance to meature the similarity between two audio signals, so we think our smoothing variants are applicable. we acknowledge that there are better evaluation metrics to measure signal quality in audio domain, such as Signal-to-Noise Ratio (SNR) and Speaker Encoder Cosine Similarity (SECS)~\cite{casanova2021sc}. It will be an interesting future work to derive certified bounds on those metrics instead of $\ell_2$-norm perturbation. Deriving certified robustness for text watermarking is more difficult, because text is not continuous like image and audio. Therefore, we can not simply add gaussian noises to watermarked texts. One way is to apply our smoothing variants in text embedding space, which is not as intuitive as in image and audio domains.

% \myparatight{Further improving certified robustness} In our experiments, as shown in Figure~\ref{figure:diff training}, we can theoretically guarantee the detection of watermark when the perturbation is $\ell_2$-norm bounded by 0.3. The size of perturbation is not large in real-world, which means that an attacker may remove the watermark without greatly degrading the image's visual quality. We acknowledge that the certified robustness of our smoothing variants inherit from HiDDeN watermarking methods~\cite{zhu2018hidden}. To further improve the robustness, we may add larger gaussian noises in adversarial training process so that we can also use larger noises in smoothing process, or design more robust image watermarking methods. 
